Improving Temporal Action Segmentation via Constraint-Aware Decoding

Temporal action segmentation (TAS) divides untrimmed videos into labeled action segments. While fully supervised methods have advanced the field, challenges such as action variability, ambiguous boundaries, and high annotation costs remain, especially in new or low-resource domains. Grammar-based approaches improve segmentation with structural priors but rely on complex parsing limiting scalability. In this work, we propose a lightweight, constraint-based refinement framework that enhances TAS predictions by integrating statistical structural priors such as transition confidence, action boundary sets, and per-class duration, that can be directly extracted from annotated data. These constraints are integrated into a modified Viterbi decoding algorithm, allowing inference-time refinement without retraining or added model complexity. Our approach improves both fully and semi-supervised TAS models by correcting structural prediction errors while maintaining high efficiency. Code is available at https://github.com/LUNAProject22/CAD

==> tables/algo_pseduo_table.tex <==
\begin{algorithm}[ht!]
\scriptsize  % Reduce font size


\KwIn{Emission probabilities $E \in \mathbb{R}^{T \times N}$, transition probabilities $P$, constraint rules $R$}
\KwOut{Optimal state sequence $\hat{Y}_{1:T}$}

\BlankLine
\tcp{Initialization}
Initialize $V[t,s] = -\infty$ for all $t,s$\;
Initialize duration tracker $D[t,s] = 0$ for all $t,s$\;
\For{$s \in R.\text{valid\_start\_actions}$}{
    $V[0,s] = \log E[0,s]$\;
    $D[0,s] = 1$\;
}

\BlankLine
\tcp{Forward Pass}
\For{$t = 1$ to $T-1$}{
    \For{each state $s$}{
        \For{each previous state $s'$}{
            \If{$V[t-1,s'] = -\infty$}{continue\;}
            
            \tcp{Check transition validity}
            \If{$s' \neq s$ and transition $(s' \to s)$ not allowed}{continue\;}
            
            \tcp{Check duration constraints}
            \If{$s' \neq s$ and $D[t-1,s']/T < R.\text{min\_duration}[s']$}{continue\;}
            
            \tcp{Calculate new duration and probability}
            \eIf{$s = s'$}{
                $d = D[t-1,s] + 1$\;
                \If{$d > R.\text{max\_duration}[s]$ or $d/T > R.\text{max\_norm\_duration}[s]$}{continue\;}
                $p = 0.9$ \tcp*{self-transition probability}
            }{
                $d = 1$\;
                $p = P[(s',s)]$ \tcp*{transition probability}
            }
            
            \tcp{Update if better path found}
            $score = V[t-1,s'] + \log p + \log E[t,s]$\;
            \If{$score > V[t,s]$}{
                $V[t,s] = score$\;
                $backpointer[t,s] = s'$\;
                $D[t,s] = d$\;
            }
        }
    }
}

\BlankLine
\tcp{Find best final state}
$s^* = \arg\max_{s \in R.\text{valid\_end\_actions}} V[T-1,s]$ subject to duration constraints\;

\BlankLine
\tcp{Backtrack to recover path}
\Return{Backtrack from $s^*$ using $backpointer$ to get $\hat{Y}_{1:T}$}\;

\caption{Constraint-based Viterbi decoding}
\label{alg:constrained_viterbi}
\end{algorithm} 


% % Alternative: Even more compact version
% \begin{algorithm}[ht]
% \footnotesize  % Even smaller font
% \caption{Constrained Viterbi Decoding (Compact)}
% \label{alg:constrained_viterbi_compact}
% \KwIn{$E \in \mathbb{R}^{T \times N}$, transition probs $P$, rules $R$}
% \KwOut{Optimal sequence $\hat{Y}_{1:T}$}

% \tcp{Initialize with valid start actions}
% $V[0,s] = \log E[0,s]$ if $s \in R.\text{start}$, else $-\infty$\;
% $D[0,s] = 1$ if $s \in R.\text{start}$, else $0$\;

% \tcp{Dynamic programming}
% \For{$t = 1$ to $T-1$}{
%     \For{$s = 0$ to $N-1$}{
%         $V[t,s] = \max_{s'} \{ V[t-1,s'] + \log P_{s' \to s} + \log E[t,s] \}$\;
%         subject to transition and duration constraints in $R$\;
%         Update $D[t,s]$ and $backpointer[t,s]$ accordingly\;
%     }
% }

% Find $s^* = \arg\max_{s \in R.\text{end}} V[T-1,s]$ with valid duration\;
% \Return{Backtrack from $s^*$ to get $\hat{Y}_{1:T}$}\;
% \end{algorithm}
